Heterogeneous Sheaf Neural Networks

Heterogeneous graphs, whose nodes and edges can belong to different types and feature spaces, arise in many real-world domains, including biology, recommendation, social networks, and computer systems. Existing heterogeneous graph neural networks typically handle this heterogeneity at the architectural level through relation-specific modules, meta-path machinery or type-aware attention, which often leads to increasingly specialised parameter-heavy designs. In this work, we propose HetSheaf, a framework for learning heterogeneous graphs through cellular sheaves. Instead of encoding heterogeneity solely in the architecture, HetSheaf represents it directly in the underlying data structure by assigning type-aware local feature spaces and learning restriction maps conditioned on node features, node types, and edge types. To support graph-level prediction, we further introduce SheafPool, a universal stalk-space readout that aggregates node representations while being invariant to local changes of basis, thereby making graph classification with sheaf networks well-defined and achieving an F1 Score up to 42 percentage points higher than mean pooling. Across a diverse suite of benchmarks (node classification, link prediction and graph classification). HetSheaf consistently achieves up to 2 percentage points higher performance (up to 94.97% Macro F1 Score on node classification and up to 99.62% on link prediction) on the Heterogeneous Graph Benchmark (HGB) framework against homogeneous (GCN, GAT, GIN, GraphSAGE), heterogeneous (R-GCN, HAT, HGT) and type-agnostic sheaf baselines, while reducing the number of parameters by up to 10$\times$.

==> sections/4_methods.tex <==
\section{Heterogeneous Sheaf Neural Networks}

\noindent\textbf{Heterogeneous Graph Setting.} We consider a heterogeneous graph~\citep{sunMiningHeterogeneousInformation2012} $\gG = (\gV,\gE,\phi,\psi)$, where $\gV$ and $\gE$ denote the sets of nodes and edges, while $\phi:\gV\to\Phi$ and $\psi:\gE\to\Psi$ are node and edge type mapping functions respectively. For an edge $e=(u,v)$, we interchangeably write its type as $\psi(e)$ or $\psi(u,v)$. Each node $u\in\gV$ is associated with a feature vector $\rvx_u$, whose dimensionality may depend on the node type. Concretely, for every type $t\in\Phi$, all nodes of type $t$, defined as $\{u \in \gV \mid \phi(u) = t\}$, share the same input dimension $d_0^t$, so that $\rvx_u \in \mathbb{R}^{d_0^{\phi(u)}}$. Unlike homogeneous graphs, where all node features are assumed to lie in a common ambient space, heterogeneous graphs naturally involve multiple feature spaces, semantic roles, and interaction patterns across node and edge types, reason for which different node types may have different feature dimensions. 

\begin{figure}[tbp]
    \centering
    \begin{subcaptiongroup}
        \includegraphics[width=0.7\textwidth]{figures/figure1.pdf}
        \phantomcaption\label{fig:metapath-gnn}
        \phantomcaption\label{fig:sheaf-pipeline}
        \phantomcaption\label{fig:hetero-sheaf}
    \end{subcaptiongroup}
    \captionsetup{subrefformat=parens}
    \caption{
        \textbf{\textsc{HetSheaf}: A Sheaf-based framework for Heterogeneous data.}
        (a) \emph{Meta-path based model.} Conventional heterogeneous GNNs typically encode heterogeneity through specialised architectural components, e.g.\ meta-path extractors or relation-aware message passing.
        (b) \emph{HetSheaf pipeline.} In contrast, \textsc{HetSheaf} captures heterogeneity directly in the data representation by inferring a cellular sheaf over the input graph. Node features are first projected into a common channel dimension, after which node stalks and restriction maps are inferred as described in \cref{sec:hetero-sheaf-predictors}. The resulting heterogeneous sheaf can then be processed by any sheaf neural architecture.
        (c) \emph{Learning heterogeneous sheaves.} The sheaf predictor enriches node features with node- and edge-type information, yielding a sheaf structure explicitly conditioned on the heterogeneous input.
    }
    \label{fig:method-diagram}
\end{figure}

\noindent\textbf{Sheaves as a Natural Representation for Heterogeneous Graphs.} Existing heterogeneous GNNs (\Cref{fig:metapath-gnn}) handle heterogeneity at the architectural level, for example through type-specific transformations, relation-dependent parameters, or meta-path-based encoders. While effective, this approach often leads to increasingly specialised and parameter-heavy designs scaling with the number of entity types, making the treatment of heterogeneity tightly coupled to the neural architecture itself. We instead take a \emph{representation-centric view}: we propose to modify the input structure to encode specific heterogeneous knowledge while maintaining topological information. The core limitation of a standard graph is that it implicitly treats node representations as living in a single shared feature space. This assumption is well aligned with homogeneous data, but becomes unnatural in heterogeneous settings, where different node and edge types may correspond to fundamentally different local spaces. Cellular sheaves address precisely this mismatch. A sheaf assigns a local vector space to each node and edge, together with restriction maps that govern how information is communicated between them. In doing so, it preserves type-specific local structure while still supporting coherent global message passing. This makes sheaves a particularly natural model for heterogeneous relational data. Rather than forcing heterogeneity to be absorbed by the architecture, we encode it directly into the underlying relational object. The role of the neural network then shifts from compensating for the limitations of the graph representation to learning over a structure that already respects the typed geometry of the data.


\subsection{\textsc{HetSheaf}: A Sheaf-based framework for Heterogeneous data}
\label{sec:hetsheaf-framework}

Motivated by this perspective, we introduce \textbf{\textsc{HetSheaf}}, a general framework for heterogeneous sheaf neural networks. Given a heterogeneous graph $\gG = (\gV,\gE,\phi,\psi)$, \textsc{HetSheaf} (\Cref{fig:sheaf-pipeline}) first preprocesses type-dependent node features into a common channel dimension, then infers a cellular sheaf whose restriction maps are conditioned on both features and type information, and finally applies a sheaf neural architecture for downstream prediction.

More formally, a heterogeneous sheaf neural network consists of three components:
\begin{enumerate}
    \item \emph{Type-aware preprocessing}, which projects type-specific input features into a shared channel space. Indeed, as each node type may have a different number of feature channels, we use a linear layer with bias for each node type to project the node features to the same number of input channels. This can be combined with the sheaf projection step of the SheafGNN to create the sheaf cochain $\rvx \in C^0(\gG, \gF)$. The modified linear layer takes in the original feature channels $f_{0}$ and outputs $df$ features as the node stalk projection. We follow \cite{lvAreWeReally2021a,zhouSlotGATSlotbasedMessage2023} to generate the input feature types by using either all of the node feature types (type-0), only the feature of the node target type (type-1) or replacing all node features as one-hot vectors (type-2). 
    \item \emph{Heterogeneous sheaf inference}, (\Cref{fig:hetero-sheaf}) which predicts restriction maps conditioned on node features and type information.
    \item \emph{Sheaf-based representation learning}, which applies a sheaf neural encoder followed by a task-specific decoder or readout. Similar to \cite{lvAreWeReally2021a}, we perform $\ell_2$ normalisation on the output embedding, $\rvo_{u} = \frac{\rvh^{(L)}_u}{\norm{\rvh^{(L)}_u}}$, where $\rvo_{u}$ is the final output embedding for a node $u \in \gV$ and $\rvh^{(L)}_u$ is the final hidden representation from the SheafGNN. For link prediction, we adapt JKNet~\citep{xuRepresentationLearningGraphs2018} to create the final embedding by concatenating the hidden representations for each layer, i.e.: $\rvo_{u} = \concat_{l=1}^{L} \frac{\rvh^{(l)}_u}{\norm{\rvh^{(l)}_u}}$.
\end{enumerate}

Let $\mathcal P$ denote the preprocessing module, $\boldsymbol{\Phi}$ the sheaf predictor, $\mathcal M$ a sheaf neural encoder, and $\mathcal D$ a downstream decoder. The overall pipeline can be written abstractly as:
\begin{align}
    \rvz_u &= \mathcal P_{\phi(u)}(\rvx_u), \\
    \gF_{u \trianglelefteq e\coloneq(u,v)} &= \boldsymbol{\Phi}(\rvz_u,\rvz_v,\phi(u),\phi(v),\psi(e)), \\
    \hat{\rvy} &= \mathcal D\!\left(\mathcal M(\gG,\gF,\{\rvz_u\}_{u\in\gV})\right).
\end{align}
The central idea is that heterogeneity is encoded into the inferred sheaf itself. Once the sheaf has been constructed, it can be processed by any sheaf-based neural architecture, including NSD \cite{bodnarNeuralSheafDiffusion2022}, Sheaf Attention Networks \cite{barberoSheafAttentionNetworks2022}, Polynomial NSD \cite{borgi2026polynomialneuralsheafdiffusion} or other sheaf variants, without requiring ad hoc heterogeneous redesign.



\subsection{Heterogeneous Sheaf Predictors, Readout, and Model Adaptations}
\label{sec:hetero-sheaf-predictors}

\noindent\textbf{Heterogeneous Sheaf Predictors.} A key ingredient of \textsc{HetSheaf} is the explicit inference of restriction maps from heterogeneous information. In standard sheaf learning, restriction maps are predicted from node features alone as $\gF_{u \trianglelefteq (u,v)} = \boldsymbol{\Phi}(\rvx_u,\rvx_v)$.
Although such a predictor may implicitly recover type-dependent behaviour, it does not explicitly exploit the typed structure available in heterogeneous graphs. We therefore parameterise the restriction maps so that the learned sheaf structure is directly conditioned on node features, node and edge types (as detailed in \Cref{fig:hetero-sheaf}):
\begin{equation}
    \gF_{u \trianglelefteq e\coloneq (u,v)}
    =
    \boldsymbol{\Phi}(\rvx_u,\rvx_v,\phi(u),\phi(v),\psi(e))
    \label{eqn:sheaf-parameterisation}
\end{equation}
Following \cite{bodnarNeuralSheafDiffusion2022}, and we consider diagonal, orthogonal, and general restriction-map families (see more details in \autoref{app:restriction_maps_impl}), and we instantiate \autoref{eqn:sheaf-parameterisation} through a \emph{family of heterogeneous sheaf predictors} that vary along two axes. The former concerns \emph{which type signals are used}: from no type information (Sheaf-NSD, where we only concatenate information relative to the node features $\rvx_u, \rvx_v$), to node-only (\textsc{HetSheaf-NE, HetSheaf-NT}) or edge-only (\textsc{HetSheaf-EE, HetSheaf-ET}) variants, up to predictors conditioned on both node and edge types (\textsc{HetSheaf-TE, HetSheaf-types}). The latter regards instead \emph{how type information is routed}: most variants use a shared MLP with type indicators as additional inputs, whereas \textsc{HetSheaf-ensemble} allocates a separate predictor to each edge type $\text{MLP}_{\psi(e)}$ , increasing expressivity at the cost of additional parameters. \Cref{fig:sheaf-predictors} summarises the predictor family, while full details and complexity analyses are deferred to \Cref{app:hetero-sheaf-predictors}.
\begin{figure}[!htbp]
    \centering
    \resizebox{0.8\textwidth}{!}{%
         \input{figures/sheaf_learners_v2}
    }
    \caption{
        \textbf{Heterogeneous Sheaf Predictors.}
        For an edge $e=(u,v)$, $\phi(u)$ and $\phi(v)$ denote node types, $\psi(e)$ denotes the edge type, $x_u,x_v$ are node features, $\|$ denotes concatenation, and $\mathrm{MLP}_{\psi(e)}$ denotes a separate MLP for each edge type.
    }
    \label{fig:sheaf-predictors}
\end{figure}

\noindent\textbf{Restriction Map Types.} A further design choice concerns how the raw output of $\boldsymbol{\Phi}$ is converted into a restriction map as in \citet{bodnarNeuralSheafDiffusion2022}. Alternatively, one may apply an attention-style post-processing step. For the general case, a row-wise softmax yields row-stochastic restriction maps, and this transformation depends only on the output of $\boldsymbol{\Phi}$, applying uniformly to all heterogeneous predictor variants:
\begin{equation}
    \gF_{u \trianglelefteq e}
    =
    \rmI_d - \mathrm{softmax}\!\left(\boldsymbol{\Phi}(\rvx_u,\rvx_v)\right)
    \label{eq:sheafan-general}
\end{equation}


\noindent\textbf{Task-specific Preprocessing and Readout}
Because different node types may have different input dimensionalities, we use a type-specific linear projection with bias to map all node features into a shared channel dimension. These projections are learned jointly with the rest of the model and can be combined with the initial stalk projection of the sheaf encoder to construct the input cochain $\rvx \in C^0(\gG,\gF)$. Following \citet{lvAreWeReally2021a,zhouSlotGATSlotbasedMessage2023}, we consider multiple feature initialisation strategies, including using all available node features, target-type-only features, and one-hot type indicators. For \emph{node classification}, we apply $\ell_2$ normalisation to the final node representation: $\rvo_u=    \frac{\rvh_u^{(L)}}{\norm{\rvh_u^{(L)}}}$, where $\rvh_u^{(L)}$ is the final hidden state of node $u$. For \emph{link    prediction}, we follow a JKNet-style strategy~\citep{xuRepresentationLearningGraphs2018} and concatenate the normalised hidden states across layers: $\rvo_u=\concat_{l=1}^{L}\frac{\rvh_u^{(l)}}{\norm{\rvh_u^{(l)}}}$. 


\noindent\textbf{Sheaf Models Adaptations.}
A key advantage of \textsc{HetSheaf} is its model-agnosticity: once a heterogeneous sheaf has been inferred through \autoref{eqn:sheaf-parameterisation}, the resulting typed geometric structure can be processed by a broad class of existing sheaf neural architectures with only minimal modifications. To demonstrate this property, we adapt both \emph{Sheaf Attention Networks} (SheafAN)~\citep{barberoSheafAttentionNetworks2022} and \emph{Polynomial NSD} (PolyNSD)~\citep{borgi2026polynomialneuralsheafdiffusion} to the heterogeneous setting. For SheafAN, we make the attention mechanism type-aware by augmenting the attention input with node-type and edge-type information:
\begin{equation}
    \Lambda_{ij} =
    \frac{
        \exp\!\left(
            \mathrm{LeakyReLU}\!\left(
                \rva^\top[
                    \rmW\rvx_i \| \rmW\rvx_j \|
                    \rve_{\phi(i)} \| \rve_{\phi(j)} \| \rve_{\psi((i,j))}
                ]
            \right)
        \right)
    }{
        \sum_{k \in \mathcal{N}_i}
        \exp\!\left(
            \mathrm{LeakyReLU}\!\left(
                \rva^\top[
                    \rmW\rvx_i \| \rmW\rvx_k \|
                    \rve_{\phi(i)} \| \rve_{\phi(k)} \| \rve_{\psi((i,k))}
                ]
            \right)
        \right)
    }.
\end{equation}
Thus, both the attention coefficients and the corresponding transport operators
$\rmP_{ij}=\gF_{i \trianglelefteq e}^{\top}\gF_{j \trianglelefteq e}$
become consistent with the heterogeneous sheaf structure. For PolyNSD, instead, we preserve the original polynomial spectral filtering scheme and apply it directly to the heterogeneous sheaf Laplacian $p(L_{\gF}) = \sum_{k=0}^{K} c_k L_{\gF}^{k}$, where $L_{\gF}$ is now induced by the type-aware restriction maps learned by \textsc{HetSheaf}. In this way, higher-order diffusion is performed directly over the heterogeneous sheaf without requiring any ad hoc redesign of the polynomial model. Full model-specific derivations and implementation details are deferred to \Cref{app:sheafan,app:polynsd}.


\textcolor{red}{TILL HERE, ALL CHECKED AND (ALMOST FINAL)}



























\section{Graph-level Readout: Universal Stalk-Space Late-token}
\label{sec:universal_stalk_space_late_token}
Graph-level prediction is substantially more delicate in sheaf models than in standard GNNs. In ordinary graph networks, node embeddings lie in a common latent space and can therefore be pooled directly. In contrast, sheaf node embeddings $\rmH_i \in \mathbb{R}^{d \times C}$ live in local stalk spaces and are only defined up to node-wise changes of basis. A valid graph readout must satisfy two requirements simultaneously: it must be permutation-invariant over nodes, and invariant under stalk-wise gauge transformations $\rmH_i \mapsto \rmG_i \rmH_i,  \rmG_i \in \mathbb{R}^{d \times d}$. Naive flatten-and-pool operations applied to sheaf neural networks violate these requirements.

To address this issue, we introduce a \emph{Universal Stalk-Space Late-token Readout}, a gauge-aware graph pooling mechanism compatible with \emph{all sheaf families}. The key idea is to canonicalise node embeddings before pooling: we first remove local $GL(d)$ distortions by per-node whitening, then resolve the residual orthogonal ambiguity via anchor-based alignment, pool the aligned stalk representations in stalk space, and finally extract an invariant graph descriptor. This yields a graph embedding that is permutation-invariant over nodes and robust to local changes of stalk coordinates. The resulting graph embedding $\rvg_g \in \mathbb{R}^C$ is then fed to a standard MLP decoder. We describe this idea here briefly and analysed further in \Cref{app:universal_stalk_space_late_token,app:universal_pooling_derivations}. 

















\begin{figure*}[t]
    \centering
    \makebox[\linewidth][c]{%
        \adjustbox{width=1.13\linewidth}{%
            \input{figures/universal_stalk_space_late_token_readout_tikz}
        }%
    }
    \caption{Universal Stalk-Space Late-token Readout.}
    \label{fig:universal-stalk-space-late-token}
\end{figure*}





















We define a graph-level readout
\begin{equation}
    \{\rmH_i\}_{i \in \gV}
    \;\mapsto\;
    \rvg_g \in \mathbb{R}^{C},
\end{equation}
that is permutation-invariant over nodes and applicable across diagonal, orthogonal, and general restriction-map families. Formally, if node embeddings are reparameterised as $\rmH_i \mapsto \rmG_i \rmH_i$, a correct readout should not depend on the particular choice of local stalk coordinates. Since direct pooling in $\mathbb{R}^{dC}$ generally fails to satisfy this property, we instead pool in stalk space after a two-stage canonicalisation.

The readout proceeds in five stages:
\begin{equation}
    \rmH_i
    \xrightarrow{\text{whiten}}
    \rmZ_i
    \xrightarrow{\text{align}}
    \widetilde{\rmZ}_i
    \xrightarrow{\text{attn pool}}
    \rmP_g
    \xrightarrow{\text{late token}}
    \widehat{\rmT}_g
    \xrightarrow{\text{energy}}
    \rvg_g.
\end{equation}

\noindent\textbf{(1) Per-node whitening.}
To remove node-wise scaling and shearing in the stalk dimension, we form
\begin{equation}
    \rmS_i = \rmH_i \rmH_i^\top + \varepsilon \rmI_d,
\end{equation}
and define whitened features
\begin{equation}
    \rmZ_i = \rmS_i^{-1/2}\rmH_i.
\end{equation}
This approximately isotropises the stalk covariance, reducing the remaining ambiguity to an orthogonal transform.

\noindent\textbf{(2) Anchor-based alignment.}
After whitening, different nodes may still be expressed in different orthogonal frames. We therefore align them to a shared learnable anchor $\rmA \in \mathbb{R}^{d \times C}$ by solving
\begin{equation}
    \rmR_i
    =
    \arg\min_{\rmR \in O(d)}
    \|\rmR^\top \rmZ_i - \rmA\|_F^2,
\end{equation}
whose solution is given by the orthogonal Procrustes transform. The aligned representations are then
\begin{equation}
    \widetilde{\rmZ}_i = \rmR_i^\top \rmZ_i.
\end{equation}

\noindent\textbf{(3) Invariant attention weights.}
To weight node contributions during pooling, we compute the channel-wise energies of the whitened embeddings:
\begin{equation}
    \rvu_i = \mathrm{diag}(\rmZ_i^\top \rmZ_i) \in \mathbb{R}^{C},
\end{equation}
which are invariant to residual orthogonal reparameterisations. A learnable scorer $s_\theta$ then produces graph-wise attention weights
\begin{equation}
    \alpha_i
    =
    \frac{\exp(s_\theta(\rvu_i))}
    {\sum_{j \in V_g}\exp(s_\theta(\rvu_j))}.
\end{equation}

\noindent\textbf{(4) Stalk-space pooling with a late token.}
The aligned stalk embeddings are aggregated directly in stalk space:
\begin{equation}
    \rmP_g = \sum_{i \in V_g} \alpha_i \widetilde{\rmZ}_i \in \mathbb{R}^{d \times C}.
\end{equation}
To increase expressivity without introducing a hub token into the encoder---which could alter message passing and exacerbate oversmoothing---we use a \emph{late, receive-only token} $\rmT \in \mathbb{R}^{d \times C}$ updated only after pooling:
\begin{equation}
    \widehat{\rmT}_g = \phi\!\left([\rmT,\rmP_g]\right),
\end{equation}
where $\phi$ is a small channel-wise MLP with layer normalisation.

\noindent\textbf{(5) Invariant graph feature extraction.}
Finally, we collapse the stalk dimension through channel-wise energies:
\begin{equation}
    \rvg_g
    =
    \mathrm{diag}(\widehat{\rmT}_g^\top \widehat{\rmT}_g)
    \in \mathbb{R}^{C},
\end{equation}
yielding a graph representation that is permutation-invariant over nodes and robust to stalk gauge variability. Full derivations, invariance arguments, and complexity analysis are deferred to \Cref{app:universal_stalk_space_late_token,app:universal_pooling_derivations,app:pooling-overhead}.




\begin{table}[!htbp]
	\centering
	\caption{\textsc{HetSheaf} Pooling ablation over graph classification. Best results per dataset in \textbf{bold}.}
	\label{tab:pooling-ablation}
    \input{tables/pooling_ablation}
\end{table}

